Audio De-identification: A New Entity Recognition Task

Named Entity Recognition (NER) has been mostly studied in the context of written text. Specifically, NER is an important step in de-identification (de-ID) of medical records, many of which are recorded conversations between a patient and a doctor. In such recordings, audio spans with personal information should be redacted, similar to the redaction of sensitive character spans in de-ID for written text. The application of NER in the context of audio de-identification has yet to be fully investigated. To this end, we define the task of audio de-ID, in which audio spans with entity mentions should be detected. We then present our pipeline for this task, which involves Automatic Speech Recognition (ASR), NER on the transcript text, and text-to-audio alignment. Finally, we introduce a novel metric for audio de-ID and a new evaluation benchmark consisting of a large labeled segment of the Switchboard and Fisher audio datasets and detail our pipeline's results on it.

==> chapters/audiodeid_discussion.tex <==
\section{Discussion}
The goal of this paper is to present the audio de-identification problem. Such presentation should contain three parts: motivation, problem definition, and a benchmark solution for others to improve.

It is easy to motivate Audio de-Identification. Health data is segregated, and no single entity has enough data to perform machine learning research on its own (moreover it is often the case that the strongest ML groups do not sit in hospitals and thus have no medical data of their own). Getting enough data to the researchers who can work on it requires de-identification of that data. The popularity of tele-medicine services, as well as the desire to record and study real interactions between patients and physicians all point to audio de-identification. We anticipate (but leave this to future work) that video de-identification, and voice de-identification (which is now not mandatory according to HIPAA) will soon follow.

Our problem definition contains both an explicit definition of what is considered as de-identification, as well as releasing a data-set to enable further research on the problem. We used the F1 metric here to conform with the text de-identification metric, but this was not an easy decision. Indeed, one can choose a metric which favors precision over recall, for two reasons: (1) A mistake in recall can be very costly, as it could potentially leak personal information. (2) even if the precision were perfect, and ML model running on the data would have to deal with words it can't decipher (as ASR isn't perfect), so bleeping out a few unnecessary words should not be terrible. As increasing recall at the expense of precision is a matter of choosing a point on the P-R curve, we ended up sticking to F1.

Finally, we presented a benchmark solution for the audio de-identification problem.  The main challenge here is to decide if this is a real benchmark or a naive solution. It is apriori difficult to estimate what is the right error rate here. A trivial lower bound is the ASR error rate, but it may be far worse. For example, one could imagine that ASR is more likely to fail on names and on other private information (addresses etc.) than on more common words, which would lead to a higher error rate. Moreover, even if ASR does not fail on the PHI but on a different word in the vicinity, it might be very difficult to identify the PHI. On the other hand, one can imagine cases in which the PHI is misunderstood, but is identified as PHI from context. Similar arguments can be made on the other types of errors, and on the interplay between them. Given that our errors are close to {\bf WE NEED TO SAY WE ARE GOOD AND CITE NUMBERS BUT I DON'T HAVE THEM IN FRONT OF ME}
